Grid Tariffs for Peak Demand Reduction: Is there a Price Signal Conflict with Electricity Spot Prices?

The electricity grid is expected to require vast investments due to the decarbonization-by-electrification trend, calling for a change in grid tariff design which provides proper incentives for reducing peak loads. However, price signals from grid tariffs could be distorted from electricity spot prices which also represents a significant of the total consumer electricity bill. This paper attempts to identify whether there is a price signal conflict between grid tariffs and spot prices. Four different grid tariff designs are compared, using a generic demand response model as part of a cost-minimizing linear program to simulate the reduction in peak load. The method is applied to metered electricity demand from 3608 consumers in Oslo, Norway. Results show that new grid tariff designs reduce peak loads by 1-4%, and that reduction in peak load is smaller when consumers are subject to electricity spot prices.

==> Chapters/Backup/Casestudy_old.tex <==
\section{Case Study \& Data} \label{sec:casestudy}

The case study and data are similar as in \cite{HofmannPreprint}, where hourly electricity load data from 3608 consumers, including 3081 household consumers and 527 commercial consumers, were used for the analysis. A visual overview of the consumers included in the case study is shown in \Cref{fig:consumeroveview}. The consumers are located at 112 different substations, under the same transformer in Oslo, Norway, and the metered data are from the period November 2020 to October 2021. In addition, historical spot prices from the price zone NO1 are collected for the same period. 
These historical data are of particular interest because the winter of 2020/2021 saw the highest measured electricity consumption in Norway.

\begin{figure}[h]
    \centering
%    \captionsetup{justification=centering}
    \includegraphics[width=0.9\columnwidth]{Floats/Figs/consumeroveview_v2.PNG}
    \caption{Overview of the consumer data and flexibility assumptions.}
    \label{fig:consumeroveview}
\end{figure}

Several cases are studied to understand the difference in achieved grid peak demand reduction, and shown in \Cref{fig:caseoverview_optimal}. They include two benchmark tests, as well as a performance analysis of the four grid tariffs described in \Cref{sec:gridtariffs}. The grid tariff (GT) case includes the test of the grid tariffs without any spot price signal. This is expanded in the grid tariff and spot price (GT+SP) case, which includes the combined price signal from each of the four grid tariffs as well as the spot price. Finally, the system optimal response (SOR) and the spot price (SP) case represent the benchmark tests. The SOR case is defined as the system's maximum ability to reduce peak load with the available flexibility, and assuming that reduction is coordinated between all consumers. The SP case is the cost minimizing response under spot prices only.

In summary the following cases are analyzed:
\begin{itemize}
    \item SOR case: System optimal response
    \item GT case: Grid tariffs only
    \item GT+SP case: Grid tariffs together with spot prices
    \item SP case: Spot prices only
\end{itemize}

\begin{figure}[h]
    \centering
%    \captionsetup{justification=centering}
    \includegraphics[width=1.0\columnwidth]{Floats/Figs/caseoverview_optimal_v3.PNG}
    \caption{Overview of the case studies.}
    \label{fig:caseoverview_optimal}
\end{figure}

\input{Floats/Tabs/GTcosts_v3}

As the cost-recovery should be similar if there is no demand response, all the cost parameters of grid tariffs are determined using backwards calculation with respect to the existing energy tariff. The cost levels are shown in \Cref{tab:GTcosts}. The load data scattered with the electricity spot price in the relevant price zone (NO1) in \Cref{fig:spotpricevsload}.  The figure shows that the price sometimes correlates well with high demand, but not always. In other words, the spot price might sometimes "interfere" with the grid tariff price signal.


==> Floats/Tabs/GTcosts.tex <==
\begin{table}[h]
\begin{tabular}{lll}
\hline
\textbf{Cost term}                                                      & \textbf{Cost level}         & \textbf{Comment}                                                                         \\ \hline
Energy term                                                             & 0.25 $\frac{NOK}{kWh}$     & Applied to all tariffs                                                                   \\
Time-of-use low                                                         & 0.25 $\frac{NOK}{kWh}$     & 22-06, always on weekends                                                                \\
Time-of-use high                                                        & 2.0 $\frac{NOK}{kWh}$      & 06-22                                                                                    \\
Time-of-use dynamic                                                     & 4.5 $\frac{NOK}{kWh}$     & 06-22, during peak load days                                                             \\
\begin{tabular}[c]{@{}l@{}}Subscribed \\ capacity cost\end{tabular}     & 1000 $\frac{NOK}{kW-year}$ & \begin{tabular}[c]{@{}l@{}}Cost per kilowatt \\ per year\end{tabular}                    \\
\begin{tabular}[c]{@{}l@{}}Sub. cap. \\ energy term\end{tabular}        & 0.25 $\frac{NOK}{kWh}$     & \begin{tabular}[c]{@{}l@{}}Cost for electricity below \\ subscription level\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Sub. cap. excess \\ energy term\end{tabular} & 1.65 $\frac{NOK}{kWh}$     & \begin{tabular}[c]{@{}l@{}}Cost for electricity \\ above subscription level\end{tabular} \\
Measured peak                                                           & 75 $\frac{NOK}{kW-month}$  & Cost for peak load per month                                                             \\ \hline
\end{tabular}
\label{tab:GTcosts}
\end{table}

==> Floats/Tabs/GTcosts_v2.tex <==


\begin{table}[h]
\begin{tabular}{llll}
\hline
\textbf{Cost term}                                                      & \textbf{Symbol} & \textbf{Cost level} & \textbf{Comment}                                                                                                  \\ \hline
Energy term                                                             & $C^{ET}$            & 0.25 $\frac{NOK}{kWh}$        & Applied to all tariffs                                                                                            \\
\begin{tabular}[c]{@{}l@{}}Time-of-use \\ static\end{tabular}           & $C^{TOU}$          & 2.0 $\frac{NOK}{kWh}$         & \begin{tabular}[c]{@{}l@{}}06-22 during winter except weekends\\ and holidays, energy term otherwise\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Time-of-use \\ dynamic\end{tabular}          & $C^{dynTOU}$        & 4.5 $\frac{NOK}{kWh}$         & 06-22, during the 10 peak load days                                                                               \\
\begin{tabular}[c]{@{}l@{}}Subscribed \\ capacity cost\end{tabular}     & $C^{sub}$          & 1000 $\frac{NOK}{kW-year}$    & \begin{tabular}[c]{@{}l@{}}Cost per kilowatt \\ per year\end{tabular}                                             \\
\begin{tabular}[c]{@{}l@{}}Sub. cap. excess \\ energy term\end{tabular} & $C^{h}$             & 1.65 $\frac{NOK}{kWh}$        & \begin{tabular}[c]{@{}l@{}}Cost for electricity above subscription \\ level, energy term when under\end{tabular}  \\
Measured peak                                                           & $C^{peak}$          & 75 $\frac{NOK}{kW-month}$     & Cost for peak load per month                                                                                      \\ \hline
\end{tabular}
\label{tab:GTcosts}
\end{table}
